Feynman categories and Representation Theory

We give a presentation of Feynman categories from a representation--theoretical viewpoint. Feynman categories are a special type of monoidal categories and their representations are monoidal functors. They can be viewed as a far reaching generalization of groups, algebras and modules. Taking a new algebraic approach, we provide more examples and more details for several key constructions. This leads to new applications and results. The text is intended to be a self--contained basis for a crossover of more elevated constructions and results in the fields of representation theory and Feynman categories, whose applications so far include number theory, geometry, topology and physics.

==> preamble.tex <==
% !TEX root = ausrevised.tex

\usepackage{cite}
\usepackage{mathtools}
\usepackage{amsmath,color}
\usepackage[v2,all]{xy}
\xyoption{2cell}
\UseTwocells
%\usepackage{graphicx}
\usepackage{amsfonts,amssymb}
%\usepackage{mathrss,a4wide}
\usepackage{mathrsfs}
%\usepackage{eufrak}
%\usepackage{mathabx}
%\usepackage{pifont}
\usepackage{leftidx}
\RequirePackage[raiselinks=false,colorlinks=true,citecolor=blue,urlcolor=black,linkcolor=blue,bookmarksopen=true]{hyperref}
% \usepackage{geometry}
%\usepackage{marginnote}
%
%\def\maybetypo#1{\marginpar{typo? maybe}{\color{red}{\bf #1}}}  % commentary!
%\def\CHANGED#1{{\color{red}{\bf #1}}}  % commentary!
%\def\ANS#1{{\color{blue}{\bf #1}}}  % Answer!
%\def\QU#1{\marginpar{\bf Question}{\color{blue}{\bf #1}}}  % question!
%\def\RMK#1{\marginpar{\color{blue}{#1}}}
%\def\CHANGED#1{}     % remove commentary!

%\usepackage[]{showkeys}
%\usepackage{refcheck}

\def\Sha{\amalg \!\!\amalg}
\usepackage{amssymb}
%\input{epsf.sty}

\usepackage{bold}
 \def\unit{\Eins}
 \def\gh{\mathbbnew{\Gamma}}
 \def\DDelta{\mathbbnew \Delta}

\catcode `\@=11
\def\numberbysection{\@addtoreset{equation}{section}
         \renewcommand{\theequation}{\thesection.\arabic{equation}}}
\numberbysection
\def\subsubsection{\@startsection{subsubsection}{3}%
  \normalparindent{.5\linespacing\@plus.7\linespacing}{-.5em}%
  {\normalfont\bfseries}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{claim}[thm]{Claim}
\newtheorem{dfprop}[thm]{Definition-Proposition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{ep}[thm]{Expectation}

\theoremstyle{definition}

\newtheorem{df}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{qu}[thm]{Question}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{cav}[thm]{Caveat}
\newtheorem{nota}[thm]{Notation}
\newtheorem{ex}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{as}[thm]{Assumption}
\newtheorem{const}[thm]{Construction}

\def\C{\mathcal C}
\def\M{\mathcal M}

\def\O{\mathcal{O}}
\def\Ab{\mathcal{A}\!\! \it b}
\def\Z{\mathbb{Z}}
\def\Q{\mathbb{Q}}
\def\Vect{\mathcal{V}\!\! \it ect}
\def\kVect{\Vect_k}
\def\dgVect{dg\mdash\kVect}
\def\cat{\mathcal{C}at}
\def\Set{\mathcal{S}et}
\def\V{\mathcal V}
\def\H{\mathscr H}
\def\E{\mathcal{E}}
\def\Mor{Mor}
\newcommand{\leftsub}[2]{{\vphantom{#2}}_{#1}{#2}}
\newcommand{\bisub}[3]{{\vphantom{#2}}_{#1}{#2}_{#3}}


\def\SSigma{$\Sigma$}


\makeatother
\newcommand{\EZDIAG}[5]{\xymatrix
@C+=2.5cm{*+[r]{#1}
\ar@(u,l)_(0.62){\displaystyle #5}[]
\ar@<1ex>^-{#3}[r]&\ar@<1ex>^-{#4}[l]#2}}


\def\del{\partial}
\def\Coop{\check\O}
\def\id{{\mathrm{id}}}
\def\hI{\hat I}
\def\HG{\H_G}
\def\PQ{\HG}
\def\HB{\H_B}
\def\SS{\mathbb{S}}
\def\ot{\otimes}
\def\odo{\otimes \dots\otimes}
\def\cdc{\cdot \ldots\cdot}
\def\kdk{,\dots,}
\def\eps{\epsilon}
%\def\unit{1\!\!1}
\def\Hbar{{\H^{bar}}}
\def\B{\mathcal{B}}
\def\rdel{\stackrel{\leftarrow}{\del}}
\def\ldel{\stackrel{\rightarrow}{\del}}
\def\Bred{\B^{red}}
\def\nn{\nonumber}
\def\I{\mathscr {I}}
\def\J{\mathscr {J}}
\def\C{\mathscr {C}}
\def\Gr{\mathcal {G}}
\def\proj{pr}
\def\Rad{\mathcal R}

\def \colim {\mathop {\rm colim}}
\def\F{\mathcal{F}}
\def\FF{\mathfrak F}
\def\fB{\mathfrak{B}}
\def\fb{\mathfrak{b}}
\def\fG{\mathfrak G}
\def\frakV{\mathfrak V}
\def\asts{{\mathcal V}}
\def\ff{\mathfrak{f}}
\def\fS{\mathfrak{S}}
\def\fs{\mathfrak{s}}
\def\fI{\mathfrak{I}}
\def\fp{\mathfrak{p}}
\def\fK{\mathfrak{K}}
\def\fL{\mathfrak{L}}
\def\fri{\mathfrak{i}}
\def\frj{\mathfrak{j}}
\def\frk{\mathfrak{k}}



\def\star{{*}}
\def\stars{{\mathcal V}}
\def\clusters{{\mathcal F}}
\def\N{\mathbb{N}}
%\newlength{\bulletwidth}
%\settowidth{\bulletwidth}{\textbf{$\bullet$}}
\def\dottree{\bullet\hskip-.35pc |\; }
\def\simpcat{{\Delta}}
\def\tn{\dottree n}

%Feynmanmacros
%\def\gh{I\hskip -3pt \Gamma}


\def\egr{\unit_{\emptyset}}
\def\nn{\nonumber}
\def\vardel{\delta}
\def\CHom{\mathcal{H}\!\it om}
\def\eps{\epsilon}
\def\G{\Gamma}
\def\arity{ar}
\def\Vect{\mathcal{V}\!\it ect}
\def\dgVect{dg\Vect}
\def\dgvect{\dgVect}
\def\gVect{\Vect^{\Z}}
\def\la{\langle}
\def\ra{\rangle}
\def\Fass{{\FF}^{Assoc}}
\def\Flie{{\FF}^{Lie}}
\def\Fprelie{{\FF}^{pre-Lie}}
\def\FFtriv{\FF^{\it triv}}


\def\Graphs{\mathcal{G}\!\it raphs}
%\def\Gr{\Agg}
\def\GGraph{{\mathcal PR}}
\def\gg{G}
\def\Ground{({\mathcal C},\otimes)}
%\def\forget{{\mathit F}}
\def\CalA{\mathcal{A}}
\def\CalC{{\mathcal C}}
\def\CalD{{\mathcal D}}
\def\CalE{{\mathcal E}}
\def\base{{B}}
\def\CalB{{\mathcal B}}
\def\CalG{{\mathcal G}}
\def\CO{{\mathcal O}}
\def\Agg{\mathcal {A}\!\it gg}
\def\Set{\mathcal {S}\!\it et}
\def\Top{\mathcal {T}\!\!\!\it op}

\def\Crl{\mathcal {C}\!\it rl}
\def\nCrl{\Crl_{\N}}
\def\pCrl{\Crl_{\mathrm planar}}
\def\pCyclic{\Cyclic_{\mathrm planar}}
\def\Cyclic{{\mathcal C}\!\it yc}
\def\opd{\mathcal{O}\!\it pd}
\def\CCyclic{\mathfrak  {C}}
\def\nCyclic{\Cyclic_{\N}}
\def\operads{{\mathfrak O}}
\def\props{{\mathfrak P}}
\def\properads{{\mathfrak P}^{ctd}}
\def\dioperads{{\mathfrak D}}
\def\modular{{\mathfrak M}}
\def\GGCrl{\GGraph\Crl}
\def\Coll{{\mathcal C}\!\it oll_{\GGraph,\Ground}}
\def\F{\mathcal F}
\def\FF{\mathfrak F}
\def\BB{\mathfrak B}
\def\GG{\mathfrak G}
\def\FD{\mathfrak D}
\def\Sk{{\mathcal S}k}
\def\one{1\!\!I}




\def\PF{{\mathcal P}_{\F}}
\def\FV{\F_{\V}}
\def\VV{\V_{\V}}
\def\FFV{\FF_{\V}}
\def\iV{\imath_{\V}}
\def\fL{\mathfrak{L}}


\def\R{{\mathbb R}}
\def\C{\CalC}
\def\Z{{\mathbb Z}}
\def\N{{\mathbb N}}
\def\G{\Gamma}

\def\del{\partial}
%\def\colim{\mathrm{colim}}

\def\FinSet{\mathcal{F}\!\it in\mathcal{S}\!\it et}
\def\FFinSet{\mathfrak{F}\!\it in\mathfrak{S}\!\it et}
\def\NCSet{\mathcal{NC}\!\it Set}
\def\FNCSet{\mathfrak{NC}\!\it Set}
\def\surj{FS}
\def\Surj{\mathfrak{FS}}
%\def\Surj{\mathcal{S}urj}
%\def\Surj{\mathfrak{S}urj}
\def\Inj{\FF\fI}
\def\inj{FI}
\def\Int{\Inj_{*,*}}
\def\FInt{\mathfrak{I}nj_{*,*}}
\def\grep{\rho_{\Gamma}}

\def\a{\alpha}


\newcommand{\op}{\mathcal}

\def\O{{\mathcal O}}
\def\P{{\mathcal P}}
\def\Sn{{\mathbb S}_n}
\def\SS{{\mathbb S}}
\def\OS{\O_{\SS}}
\def\Snp{\SS_{n+}}
\def\Endo{{\mathcal E}nd}

\def\fSet{{\mathcal FS}et^{bij}}

\def\Op{\O^{\oplus}}
\def\sOp{s\O^{\oplus}}
\def\OSp{\O^{\oplus}_{\SS}}
\def\OSpp{\O^{\oplus}_{\SS_+}}

\def\form{\la \; ,\; \ra}
\def\Gbracket{\{\;\bullet\;\}}
\def\Liebracket{[\;\circ\;]}
\def\cLiebracket{\{\;\odot\;\}}
\def\odo{\otimes \cdots \otimes}
\def\K{\mathfrak K}
\def\crl{*}
\def\coll{col}

\def\RForest{{\mathcal RF}or}
\def\Forest{{\mathcal F}or}
\def\IOForest{{\mathcal F}or^{i/o}}
\def\Dirgraph{{\mathcal DG}}
\def\Gra{\mathfrak{G}ra}
\def\day{\circledast}

\def\wt{\mathrm{wt}}
\def\deg{\mathrm{deg}}

\def\kill{trun}
\def\leaf{leaf}

\newcommand\ccirc[2]{\, \leftsub{#1}{\circ}_{#2}}
\def\scirct{\ccirc{s}{t}}
\newcommand\Sccirc[2]{\, \leftsub{#1}{\circ}_{#2}^{S^1}}
\newcommand\mge[2]{\, \leftsub{#1}{\boxminus}_{#2}}



\newcommand{\obj}{\operatorname{Obj}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\drpullback}[1][dr]{\save*!/#1-1.2pc/#1:(-1,1)@^{|-}\restore}


\newcommand{\ds}{\displaystyle}

\def\t{\tau}
\def\con{con}
%\def\{\ast}
%genop stuff
%\def\ast{{*}}
\def\V{\asts}
\def\asts{{\mathcal V}}
\def\F{\clusters}
\def\clusters{{\mathcal F}}
\def\isoclusters{Iso(\F)}
\def\Ab{{\mathcal Ab}}
\def\gAb{g\Ab}
\def\CalG{{\mathcal G}}
\def\opcat{{\mathcal O}\!\it ps}
\def\Fops{\F\text{-}\opcat}
%\def\op{{\mathcal O }p}
\def\smodcat{{\mathcal M}\!\it ods}
\def\Vmods{\V\mdash\smodcat}
\def\mods{\smodcat}
\def\forget{\mathit {forget}}
\def\free{\mathit {free}}
\def\T{{\mathbb T}}
\def\I{{\mathcal I}}
\def\D{\mathcal D}

\def\inthom{\underline{\Hom}}
\def\Aut{\it{Aut}}
\def\Iso{\it{Iso}}

%\def\feynman{{\mathbb F}}

\def\oper{\mathcal{O}\!\it p}
\def\opers{\opcat}

\def\ta{\twoheadrightarrow}

\def\trivial{\mathcal{T}}
\def\triv{\underline{\mathbf{1}}}

\newcommand{\X}{{\mathcal X}}
\newcommand{\Y}{{\mathcal Y}}

\def\bl#1{\textcolor{blue}{#1}}
\def\rd#1{\textcolor{red}{#1}}
\def\mmm#1{\textcolor{magenta}{#1}}

\def\length{l}
\def\weight{wt}

%%%%%%new
\def\Bquot{\B_\Q^{quot}}
\def\Hquot{\H_\Q^{quot}}
\def\epsquot{\eps^{quot}}
\def\Deltaquot{\Delta^{quot}}
\def\etaquot{\eta^{quot}}

\def\Bred{\B^{red}}
\def\Hred{\H^{red}}
\def\epsred{\eps^{red}}
\def\Deltared{\Delta^{red}}
\def\etared{\eta^{red}}

\def\Biso{\B^{iso}}
\def\Hiso{\H^{iso}}
\def\epsiso{\eps^{iso}}
\def\Deltaiso{\Delta^{iso}}
\def\etaiso{\eta^{iso}}

\def\otb{\leftsub{*}\otimes_*}

\def\ops{\opcat}
\def\dashops{\text{-}\ops}
\def\dashopcat{\dashops}
\def\op{op}

\def\FFdeco{\FF_{{\rm dec}\O}}
\def\Fdeco{\F_{{\rm dec}\O}}
\def\Vdeco{\V_{{\rm dec}\O}}
\def\ideco{\imath_{{\rm dec}\O}}

\def\clr{\mathrm{c}}
\def\lab{\mathrm{lab}}
\def\bs{\boldsymbol{ \sigma}}
\def\be{\boldsymbol{\imath}}

\def\un{\underline{n}}
\def\um{\underline{m}}
\def\uone{\underline{1}}
\def\dec{\mathrm{dec}}

\def\fopcatc{\F\text{-}\opcat_C}
\def\fopcat{\F\text{-}\opcat}


 %------------------------------------------------------------------------------------------------------
 %Ben defs

 \def\FT{\mathsf{FT}}
 \def\fops{\F\text{-}\opcat}
 \def\foddops{\F^{odd}\text{-}\opcat}
 \def\fopsc{\F\text{-}\opcat_\C}
 \def\vmods{\V\text{-}\smodcat}
 \def\vmodsc{\V\text{-}\smodcat_\C}
 \def\vseq{\V\text{-}\text{Seq}_\C}

 \def\Cobar{\Omega}
 \def\Bar{\mathsf{B}}
 \def\tensor{\otimes}
 %\def\Top{\n{Top}}
 %\def\dgvect{\textbf{dg.Vect}_k}
 \def\fopst{\F\text{-}\opcat_{\Top}}

 \newcommand{\kf}{\mathbb{K}}
% \newcommand{\id}{\mathbb{I}}

 \newcommand{\xycirc}[2]{\leftsub{#1}{\circ}_{#2}}
 \newcommand{\oxycirc}[2]{\leftsub{#1}{\ocirc}_{#2}}
 \newcommand{\ocirc}{\bar{\circ}}
 \newcommand{\fr}{\mathfrak}
 \newcommand{\lrtimes}{\bowtie}
 \newcommand{\tdt}{\tensor\dots\tensor}
% \newcommand{\cdc}{,\dots,}
 \newcommand{\fdops}{\F\text{-}\opcat_\mathcal{D}}
 \newcommand{\eops}{\mathcal{E}\text{-}\opcat_\mathcal{C}}

 \newcommand{\vemods}{\V_\fr{E}\text{-}\smodcat_\mathcal{C}}
 \newcommand{\vfmods}{\V_\FF\text{-}\smodcat_\mathcal{C}}

 \newcommand{\adj}[4]{#1\negmedspace: #2\rightleftarrows #3:\negmedspace #4}
\def\sign{\rm sign}
\def\sds{(\sigma\Downarrow\sigma')}
\def\g{\gamma}
\mathchardef\mdash="2D
\newcommand\RK[1]{\marginpar{\flushleft\bl{ #1}}}
\def\Gpd{\mathscr G}

%%Operads
\def\Assoc{\it Assoc}
\def\Ass{\Assoc}
\def\CycAssoc{\it CycAssoc}
\def\CAss{\CycAssoc}
\def\ModAssoc{\it ModAssoc}
\def\ModAss{\ModAssoc}
\def\gcp{{+\it gcp}}
\def\hyp{{\it hyp}}
\def\rt{\it rt}
\def\dec{{\rm dec}\;}
\def\red{{\it red}}

%\def\pCrl{\V\mdash\Crl_{(\F\downarrow \V)}}
\def\pCrl{\Crl_{\FF^+}}
\def\pAgg{\Agg_{\FF^+}}
\def\pO{\operads_{\FF^+}}
\def\Obj{\it Obj}
\def\Mor{\it Mor}
\def\A{\CalA}
\def\pp{\mathfrak{p}}
%\def\FFcyc{\mathfrak{C}\it \!\! yc}
\def\final{\trivial}
\def\Fe{\FF} 

\def\CObj{\mathcal{O}\!\!\it bj}
\def\CMor{\mathcal{M}\!\!\it or}
\def\IV{\mathcal{I}_V}

